Cost-efficient Data Acquisition on Online Data Marketplaces for Correlation Analysis

Incentivized by the enormous economic profits, the data marketplace platform has been proliferated recently. In this paper, we consider the data marketplace setting where a data shopper would like to buy data instances from the data marketplace for correlation analysis of certain attributes. We assume that the data in the marketplace is dirty and not free. The goal is to find the data instances from a large number of datasets in the marketplace whose join result not only is of high-quality and rich join informativeness, but also delivers the best correlation between the requested attributes. To achieve this goal, we design DANCE, a middleware that provides the desired data acquisition service. DANCE consists of two phases: (1) In the off-line phase, it constructs a two-layer join graph from samples. The join graph consists of the information of the datasets in the marketplace at both schema and instance levels; (2) In the online phase, it searches for the data instances that satisfy the constraints of data quality, budget, and join informativeness, while maximize the correlation of source and target attribute sets. We prove that the complexity of the search problem is NP-hard, and design a heuristic algorithm based on Markov chain Monte Carlo (MCMC). Experiment results on two benchmark datasets demonstrate the efficiency and effectiveness of our heuristic data acquisition algorithm.

==> extension.tex <==
\section{Discussion}

\subsection{Top-k purchase recommendations}

\subsection{Privacy}

The join is different from record linkage.

\nop{
How to extend the algorithm to cover the case that involve purchase of more than 2 attributes, Say a customer tries to purchase 4 attributes, none of two appearing in the same dataset?  

A more interesting data purchase problem is when there are more than two attributes to join, and these attributes reside in different datasets. 
In specific, let $S_1\in D_1$, $S_2\in D_2$, $\dots$, $S_k\in D_k$ be the attributes to link via data purchase, where $k>2$. 
There exists a wide range of application of this problem in practice. For example, the homeland security department benefits from linking the residence address (from bank dataset), vehicle plate number (from DMV dataset), and phone call history (from wireless service provider) to complete the information of potential terrorists.

In this problem, we are interested in discovering an affordable join path $P$, i.e., $p(P)\leq B$, that (1) connects the $k$ attributes; (2) maximizes the objective value per Equation \ref{eqn:of}. 
If we take the perspective of the join graph, as $P$ connects multiple nodes, $P$ is equivalent a spanning tree of the target attributes. 
To solve the problem, we take the heuristic approach that first discovers the set of shortest paths, i.e., the minimum spanning trees ($MST$s), and then obtains the one with the maximum objective value. 
It is worth noting that in consistency with Theorem \ref{th:mono} and \ref{th:2attribute}, for each dataset, we only consider 2-attributes to build the join path. 

In the first step, to enumerate all the $MST$s, we adapt the state-of-the-art approach \cite{yamada2010listing}, which yields $O(xm\log n)$ time complexity, where $x$ is the size of the $MST$, $m$ is the number of edges, and $n$ is the number of nodes. 
The algorithm \cite{yamada2010listing} works by taking an $MST$ $T$ as input, and trying to replace every edge in $T$ with another edge to keep the new tree connected.
In our problem, $x$ is a value in the range of $[k-1, N]$, as the size of the $MST$ can be as small as $k-1$, but as large as $N$ (need to include all the candidate datasets to connect the target attributes). While $n=\sum_{i=1}^N \binom{m_i}{2}$, because we may include any 2-attributes in the $MST$.
We must admit that when the join graph is densely connected, i.e., the candidate datasets share a large fraction of common attributes, the time complexity to generate all $MST$s might be prohibitively expensive. 
}


==> single-data-purchase.tex <==
\subsection{Single-dataset Purchase}
\subsubsection{Problem Statement}
\label{sc:ps}
As single-dataset purchase is different from multi-dataset purchase for no join will be considered, we give a separate problem statement for single-dataset purchase.
Given a relational dataset $D$ that has $m$ attributes $\mathcal{A}=\{A_1, \dots, A_m\}$, we consider the data consumer who has a budget $B$ that cannot afford purchasing $\mathcal{A}$ (i.e., $B<p(\mathcal{A})$). Therefore, the consumer would like to buy a subset of attributes $X\subseteq \mathcal{A}$ that has the best data utility. There are several aspects of data utility, which inlcudes but not limits to data quality and data size. In our case, {\em size} is defined as the number of purchased attribtutes as we only allow vertical purchase. More data would usually mean more information, therefore the buyer would like to buy as much data as he can under the budget constraint. Data quality is a more complex measurement of data utility. In our case, we consider two aspects of data quality: one is the error rate of the purchased data set calculated by $g_3$ error, another is the proportion of {\em useful} attributes. Formally, the definition of useful attribute is:
\begin{definition}
We say an attribute $A$ is {\em useful} if there exits a minimal functional dependency $F: X \rightarrow Y$ s.t:
\begin{enumerate}
\item $A\in {X\cup Y}$
\item ${X\cup Y}\subseteq S $, where $S$ is the candidate attribute set
\end{enumerate} 
\end{definition}
In this way, the objective of the buyer is to maximize the size, minimize the error, and maximize the proportion of {\em useful} attributes of the purchased data set.   
As this is a multi-objective (or multi-criteria) optimization problem, we combine the three objective functions into one {\em objective function}
 \[F(X) = (1 - error(X))  + a * \frac{|X|}{m} + \frac{|U|}{|X|}\]
, where $a$ is an amplification factor, $m$ is the number of the attributes of $D$, $|U|$ denotes the number of {\em useful} attributes, and $|X|$ denotes the number of attributes of $X$, e.g. purchased attributes. In particular, if an attribute appears in multiple approximate functional dependencies, which is highly likely to happen, it will be counted multiple times in  $|U|$.
We use $\frac{|X|}{m}$ instead of $|X|$ to make sure all three parts of the objective function are in the domain [0, 1]. However, as $m$ will be different and can vary in a large range for different data sets, while $error(X)$ will always be in the domain $[0, \theta]$, where $\theta$ is the given threshold for a relationship among attributes to be considered as an {\em approximate functional dependency}, we multiply $\frac{|X|}{m}$ by an amplification factor $a$. As the maximum range of $error(X)$ is $\theta$, $a$ is defined as $a = m * \theta$ . In this way, we ensure that different parts in the objective function play a similar role.

Formally, we define the single-dataset purchase problem as following:
\begin{equation}
\label{eqn:of}
\begin{aligned}
& \underset{X\subseteq \mathcal{A}}{\text{Maxmize}}
& &F(X) = (1 - error(X))  + a * \frac{|X|}{m} + \frac{|U|}{|X|}, 
\\
& \text{Subject to}
& & p(X) \leq B. 
\end{aligned}
\end{equation}
There is monotone property for $g_3$ error of AFD and quality of a given dataset. However, there is no monotone property for the objective function.
Thus we can reduce the {\em size-constrained non-submodular minimization} (SCNM) problem to the BCQD problem in polynomial time.
As the SCNM problem is NP-hard \cite{kawahara2015approximate, nagano2011size}, the BCQD problem is NP-hard. 
\subsubsection{Heuristic Approach}
\label{sc:heuristic}
As the BCQD problem is NP-hard, we design a heuristic algorithm to solve the problem. The algorithm is explained in details below:

Given a dataset of $m$ attributes, we design the following algorithm to heuristically pick samples from the $2^m-1$ attribute sets, and return the one that comes with the highest objective value. 
In specific, we adapt the the Markov chain Monte Carlo method \cite{robert2010introducing,gilks1995markov} and follow the Metropolis-Hastings algorithm \cite{chib1995understanding} to design Algorithm \ref{alg:mcmc}. For any attribute set $X\subseteq \mathcal{A}$, let $f(X)$ denote the objective value of $X$. The key idea is to pick affordable attribute set with the probability proportional to $f(X)$. In other words, the higher objective value an attribute set $X$ has, the more likely we sample $X$. Therefore, we are able to discover the affordable attribute set of the best utility with a high probability.

\begin{algorithm}
\caption{MCMC()}
  \begin{algorithmic}[1]
	\REQUIRE A set of attributes $\mathcal{A}=\{A_1, \dots, A_m\}$, the budget $B$, the number of attribute sets to generate $\ell$; 
	\ENSURE Randomly generate a set of attribute sets. 
	\STATE{Randomly generate an affordable attribute set $S^{(0)} \subseteq \mathcal{A}$;}
	\FOR{$i=1$ to $\ell$}
		\STATE{Let $C(S^{i-1})=\{A|A\in S^{(i-1)}\ or \ A\in \mathcal{A}\setminus S^{(i-1)},\  p(S^{(i-1)}\cup \{A\})\leq B\}$}
		\STATE{Randomly pick an attribute $A\in C(S^{(i-1)})$ in a uniform way;}
		\IF{$A\in S^{(i-1)}$}
			\STATE{$S^{(i)}=
				\begin{cases}
					S^{(i-1)} \setminus \{A\} & with\  probability\ \rho(A, S^{(i-1)})\\
					S^{(i-1)} & with\  probability\ 1-\rho(A, S^{(i-1)})
				\end{cases}			
			$
			where $\rho(A, S^{(i-1)})=min\{\frac{f(S^{(i-1)} \setminus \{A\})|C(S^{(i-1)})|}{f(S^{(i-1)})|C(S^{(i-1)} \setminus \{A\})|}, 1\}$
			}		
		\ELSE
			\STATE{$S^{(i)}=
				\begin{cases}
					S^{(i-1)} \cup \{A\} & with\  probability\ \varrho(A, S^{(i-1)})\\
					S^{(i-1)} & with\  probability\ 1-\varrho(A, S^{(i-1)})
				\end{cases}			
			$
			where $\varrho(A, S^{(i-1)})=min\{\frac{f(S^{(i-1)} \cup \{A\})|C(S^{(i-1)})|}{f(S^{(i-1)})|C(S^{(i-1)} \cup \{A\})|},1\}$
			}		
		\ENDIF
	\ENDFOR	
	\STATE{Pick the attribute set $S^*$ with the maximum $f(S^*)$} 
\end{algorithmic}
\label{alg:mcmc} 
\end{algorithm}

In Algorithm \ref{alg:mcmc}, we first generate an attribute set $S^{(0)}$ such that such that $p(S^{(0)})\leq B$. In line 3, we define the candidate attribute set of $S^{(i-1)}$ as the set of attributes which can be excluded from it, or can be added to it and the price is still within the budget. 
In line 4, we uniformly and randomly generate an attribute from $C(S^{(0)})$. In other words, the candidate-generating density function of the Metropolis-Hastings algorithm is 
\[
  q(Y|X) = \left\{
  \begin{array}{lr}
    \frac{1}{|C(X)|} & \text{if } Y=X\cup\{A\}, \text{ and } A\in C(X)\setminus X \\
    \frac{1}{|C(X)|} & \text{if } Y=X\setminus\{A\}, \text{ and } A\in X \\
    0 & otherwise
  \end{array}
  \right.
\]
Next, we generate the next sample attribute set $S^{(i)}$ in line 5-9. It is guaranteed that the attribute sets are generated with the probability of $f(X)$. In line 11, we return the attribute set $S^*$ from the samples that has the largest objective value.

The time complexity of ths algorithm mainly comes from the calculation of the exact error rate of a given data set, $g_3(X)$, which is $O(mn^2)$, where $m$ is the number of attributes of this data set and $n$ is the number of records.
The total time complexity of this algorithm is $O(lmn^2)$, where $l$ is the number of sample sets. For a given data set, $m$ and $n$ are determinate. However, $l$ can be changed to meet different requirements. Later in the experiment part we will show that even with a small $l$, the results can be of high quality. Thus this heuristic algorithm is efficient.



